Pose and Shape Estimation with Discriminatively Learned Parts

We introduce a new approach for estimating the 3D pose and the 3D shape of an object from a single image. Given a training set of view exemplars, we learn and select appearance-based discriminative parts which are mapped onto the 3D model from the training set through a facil- ity location optimization. The training set of 3D models is summarized into a sparse set of shapes from which we can generalize by linear combination. Given a test picture, we detect hypotheses for each part. The main challenge is to select from these hypotheses and compute the 3D pose and shape coefficients at the same time. To achieve this, we optimize a function that minimizes simultaneously the geometric reprojection error as well as the appearance matching of the parts. We apply the alternating direction method of multipliers (ADMM) to minimize the resulting convex function. We evaluate our approach on the Fine Grained 3D Car dataset with superior performance in shape and pose errors. Our main and novel contribution is the simultaneous solution for part localization, 3D pose and shape by maximizing both geometric and appearance compatibility.

==> tex/intro.tex <==
\begin{figure*}\label{fig:highlight}
        \centering
        \includegraphics[width=\textwidth]{figures/highlight.pdf}
             \caption{Single image car pop-up: Description of our method}\label{fig:animals}
\end{figure*}

==> tex/training.tex <==
\subsection{Local Appearance Model}{\label{sec:discriminate}}
Our object shape model is represented by a collection of 3D shape landmarks. During training, we learn a mixture of discriminative parts to model the 2D appearances of each landmark. In order to prune weak classifiers and reduce inference time, a subset of discriminative parts are selected based on their quality of detection in 2D and the joint coverage of the object shape model in 3D.

\subsubsection{Learning the appearance of Landmarks}
One of the main challenges in object pose estimation rises from the fact that due to perspective transform and self occlusions, even the same 3D position of an object has very different 2D appearances in the image observed from different viewpoints. We tackle this problem by learning a mixture of discriminative classifiers for each landmark to capture the variety in appearance.

Given a training set $D$, each training image $I_i \in D$ is associated with the 3D landmarks of the object $S \in \mathbb{R}^{3 \times p}$, and their 2D projections annotated in the image $L_i \in \mathbb{R}^{2 \times p}$ and visibility $V_i \in \{0,1\}^p$.

\textbf{Bootstrapping by clustering.} For each 3D landmark $k \in \{1, \dots, p\}$, in training image $I_i$, we extract an $N \times N$ image patch centered at its 2D locations $L_{ik}$ if it is visible $V_{ik} = 1$, assuming the images are resized such that the object is at the same scale. We denote the HOG feature of the patch as $\phi(L_{ik})$. The positive training features for the landmark $k$ is thus $\{\phi(L_{ik}) | V_{ik} = 1\}$. The negative training features $\phi(L_{\textbf{bg}})$ are HOG features of randomly extracted patches that does not have overlap with the object. Previous works have shown that whitened HOG achieves better clustering results. We adopt the same approach to first transform each feature vector into whitened space, termed whitened HOG (WHO):
\begin{align}
\textbf{WHO}[\phi(L_{ik})] = 
\Sigma^{-1/2}(\phi(L_{ik}) - \overline{\phi(L_{\textbf{bg}}}))
\end{align}
Where $\Sigma$ is the shared covariance matrix computed from both positive and negative features and $\overline{\phi(L_{\textbf{bg}})}$ is the mean of all negative features. Then we cluster the whitened features of each landmark $k$ into $m$ clusters using K-means. Let latent variable $c_{ik} \in \{1,\dots,m\}$ be the component assignment for each feature. A filter $W_{kc}, c \in \{1,\dots,m\}$ is a linear classifier learned for each cluster $c$ of a landmark $k$, using linear discriminant analysis,
\begin{align}
W_{kc} = \Sigma^{-1}(\overline{\phi(L_{ik})} - \overline{\phi(L_{\textbf{bg}}})), \; \forall c_{ik} =&\; c
\end{align}
The discriminative model for each landmark is thus a mixture of filters with $c$ components.

\textbf{Landmark responses in the image.} Let $\mathbf{x} = (x,y,l)$ be the position $(x,y)$ in the $l$-th level (scale) of an image pyramid. The space of all locations in the image pyramid is denoted as $\mathcal{X}$. The learned filters are applied in a sliding-window fashion to each location $\mathbf{x}$ in the image pyramid. The response of the landmark $k$ at a given location $\mathbf{x} \in \mathcal{X}$ is the max response over all its $c$ components:
\begin{align}
score_k(\mathbf{x}) = \max_c \{W_{kc} \cdot \phi(\mathbf{x})\}
\end{align}

\textbf{Latent update 2D location and classifier weights.} Due to annotation and clustering error, training patches may not be perfectly aligned. Such misalignment results in inferior detector performance. We introduce another latent variables for each training patch, $r_{ik}$ for relative center location to the annotated landmark location $L_{ik}$. To train a better classifier, we use the classifiers learned from clustering WHO to reposition the patch center in the neighborhood $\Delta(L_{ik})$ of $L_{ik}$ and update $c_{ik}$ and $r_{ik}$ as
\begin{align*}
\mathbf{x}^*_{ik} =&\; \text{argmax}_{\mathbf{x} \in \Delta(L_{ik})} score_k(\mathbf{x})\\ 
c_{ik} =&\; \text{argmax}_{c} \{W_{kc} \cdot \phi(\mathbf{x}^*_{ik})\}\\
r_{ik} =&\; \mathbf{x}^*_{ik} - L_{ik}
\end{align*}
The classifier weights are then retrained as
\begin{align}
\widehat{W}_{kc} = \Sigma^{-1}(\overline{\phi(L_{ik}+r_{ik})} - \overline{\phi(L_{\textbf{bg}}})), \; \forall c_{ik} =&\; c
\end{align}

Each patch mixture is retrained by linear SVM and negative examples are chosen via hard negative mining as in \cite{felzenszwalb2010object}.


Figure \ref{fig:latent} shows the filter learned from clustering and after several iterations of latent update. 


\begin{figure*}[!t]
\centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/LDA_001_002.jpg}
        \caption{clustering WHO}
        \label{fig:cluster}
    \end{subfigure}
    %add desired spacing between images, e. g. ~, \quad, \qquad etc.
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/LDA_001_002_latent_1.jpg}
        \caption{iteration 1}
        \label{fig:itr1}
    \end{subfigure}
    %add desired spacing between images, e. g. ~, \quad, \qquad etc.
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/LDA_001_002_latent_2.jpg}
        \caption{iteration 2}
        \label{fig:itr2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/LDA_001_002_latent_3.jpg}
        \caption{iteration 3}
        \label{fig:itr3}
    \end{subfigure}
    \caption{The average training patches and learned filter for a component of a landmark on the car wheel after each iteration are shown. Filters learning are bootstrapped by clustering. The latent update procedure update the center position and scale for each training patch by detecting the patches in the local region of the 2D landmark, and retrain the filters using better aligned training patches. The procedure results in more concentrated weights in learned filters.}
    \label{fig:latent}
\end{figure*}

\subsubsection{Discriminative Landmarks Selection}
Seeking a compact representation of the object, we try to select only a subset of discriminative landmarks $S_D$ among all 3D landmarks $S$. We want the selected landmarks $S_D$ to be both discriminative in the image and have a good spatial coverage of the object shape model in 3D. The selection problem is formulated as \textbf{facility location problem},
\begin{align}\label{eq:facility}
\min_{y_u, x_{uv}} ~~ & \sum_u c_{u} y_{u} + \lambda \sum_{uv} d_{uv} x_{uv} \\
\st ~~ & \sum_v x_{uv} = 1,\\
& x_{uv}  \le y_v, ~~~~~~~~~~~~~~~~ \forall u, v, \\
& x_{uv}, y_u \in \{0,1\}, ~~~~~ \forall u, v.
\end{align}
where binary variable $y_u$ is 1 if landmark $u$ is selected, binary variable $x_{uv}$ is $1$ if landmark $u$ is suppressed by landmark $v$, $c_u$ is the cost of selecting landmark $u$, and $d_{uv}$ is the cost of landmark $v$ covering landmark $u$. $\lambda$ balance the ratio between unary costs and binary costs. 

The cost $c_u$ for a landmark $u$ should be lower if the landmark is more discriminative. We model the discriminativeness by evaluating the Average Precision of detecting each landmark. For any landmark $u$, we preform detection in the training set $S$ to generate a list of bounding box hypothesis $B_u$, a bounding box hypothesis $b \in B_u$ is considered as true positive if the ground truth location $L_{iu}$ is covered by it. Let the computed AP for landmark $u$ be $AP_u$, we set $c_u = 1 - AP_u$. The cost of suppressing other landmarks are set to be the euclidean distance between landmarks in 3D, i.e., $d_{uv} = ||S_u - S_v||_2$.
% All locations cost should be positive. Thus, we set $c_u$ to be  $-\textbf{mean}_i\{score_u(L_{iu} + r_{iu})\} + C, \forall I_i \in D$, the negation of average max response of landmark $u$ on the training images at its latent position, where $C$ is a constant to ensure all $c_u > 0$.
The minimization problem \ref{eq:facility} is a Mixed Integer Programming (MIP) problem, which is known to be NP-hard. But a good approximation solution can be obtained by relaxing the integer constrains to be $x_{uv} \in [0,1], ~ y_{u} \in [0,1]$ and solve the relaxed Linear Programming problem and threshold the solution.

\begin{figure}
\label{fig:selection}
\includegraphics[width=0.5\textwidth]{figures/landmarkSelection.jpg}
\caption{Visualization of the landmark selection output. All 256 landmark of a car are shown. The color represents the Average Precision(AP) of the landmarks, red means higher AP and blue means lower AP. The size of the landmark represents the selection, the bigger ones are selected via the MIP optimization and the smaller ones are not selected.}
\end{figure}


\subsubsection{Modeling Landmarks Localization Uncertainty}
A covariance matrix $\Sigma_k$ is estimated for each landmark $k$ from latent variables $r_{ik}$, to model the uncertainty of the detected landmark position $\mathbf{x}^*_{ik}$  relative to the ground truth. 










